Industry Scale Semi-Supervised Learning for Natural Language Understanding

This paper presents a production Semi-Supervised Learning (SSL) pipeline based on the student-teacher framework, which leverages millions of unlabeled examples to improve Natural Language Understanding (NLU) tasks. We investigate two questions related to the use of unlabeled data in production SSL context: 1) how to select samples from a huge unlabeled data pool that are beneficial for SSL training, and 2) how do the selected data affect the performance of different state-of-the-art SSL techniques. We compare four widely used SSL techniques, Pseudo-Label (PL), Knowledge Distillation (KD), Virtual Adversarial Training (VAT) and Cross-View Training (CVT) in conjunction with two data selection methods including committee-based selection and submodular optimization based selection. We further examine the benefits and drawbacks of these techniques when applied to intent classification (IC) and named entity recognition (NER) tasks, and provide guidelines specifying when each of these methods might be beneficial to improve large scale NLU systems.

==> sections/old/background.tex <==
\label{background}
Self-labeling techniques are capable of providing large improvements in model performance with little effort, which could play a crucial role in large scale systems in industry. In self-labeling, we assume an input space $\mathcal X$, a label space $\mathcal Y$, and model $f$ which given an input $\mathbf{x} \in \mathcal X$ its output corresponds to the probability distribution over labels according to the model. More formally, the probability of a label $y$ given a model $f$ and input $\mathbf{x}$ can be expressed as $\Pr(Y=y | X=\mathbf{x}, f)$, where $Y$ and $X$ are random variables corresponding to labels and inputs.

There are two main strategies that are often used in self-labeling methods: hard-labeling, and soft-labeling. In hard-labeling, each unlabeled input $\mathbf{x}_u$ is assigned one specific label, $\hat y$, specifically 

\begin{eqnarray}\label{eqn:vat_kl}
    \hat{y} = \underset{y \in \mathcal{Y}}{\arg\max} \Pr(Y=y | X=\mathbf{x}_u,f),
\end{eqnarray}

On the other hand, in soft-labeling, each input considers the full distribution $\Pr(Y | X=\mathbf{x}_u,f)$.

In hard-labeling family, pseudo-labeling (PL) is one of the most commonly used methods and has been successfully applied to several NLP tasks, including parsing and word sense disambiguation \cite{yarowsky1995unsupervised,mcclosky2006effective}. While earlier research often took the straightforward pseudo-labeling approach, more recent studies have explored soft-labeling as an alternative \cite{parthasarathi2019lessons,liu2019improving,aguilar2020knowledge}. Inspired by Knowledge Distillation (KD) \cite{hinton2015distilling}, where a student model is trained based on a previously trained teacher model, it is hypothesized that leveraging the probability distribution over all labels provides more information than assuming a definitive label belonging to one particular class, thus the knowledge transfer between teacher and student could be more effective.  

In addition to KD, virtual adversarial training (VAT) and cross-view training (CVT) are two highly successful self-labelling approaches in recent years, and have achieved state-of-the-art performance on various academic benchmarks, including text classification, named entity recognition, and dependency parsing\cite{vat,cvt,vat_classification}. 

In this study, we conduct comprehensive experiments and analysis of these commonly used SSL approaches, and discuss their pros and cons in the industry setting. 

==> sections/old/datasets.tex <==
\label{datasets}

\subsection{Commercial Virtual Assistant Data Sets}
NLU products or applications in the industry are often operating with data in the scale of millions. To test different SSL techniques in web scale applications, first we employ data sets collected from a commercial NLU system. 

Four applications domains are selected for experimentation, Communication, Music, Notifications and ToDos. In this paper, we explore two types of natural language understanding (NLU) tasks: Intent Classification (IC) and Named Entity Recognition (NER). Because different application domains could have drastically different speech patterns, we train and evaluate the IC/NER models for each application domain independently. For example, the NER model for Music domain will be trained to identify music related entities such as Artist, Song and Album, while the NER model for Communication domain will focus on identifying entities such as Name and Phone Number. 

Data set generation is carried out for each domain independently. First, we collect and annotate data for a domain. The annotation is carried out for both IC and NER tasks, respectively. Then we select a subset of the data, keep the unique utterances and split into train/dev/test partitions, each with 50k unique utterances. We use stratified sampling during the data set creation to make sure that train, dev and test sets all contain the same distribution over intents. Train and dev data sets are employed during supervised and semi-supervised model training, while all models are evaluated on the test sets. 


\subsubsection{SSL Data Pool}

To evaluate and compare different SSL techniques, we create an unlabelled data pool for each application domain respectively, which contains relevant data for the target domain. To generate this data pool for a domain, we train a LSTM-based binary classifier as a data selector. The training data for the data selector is the combination of the size 50k training sets from each domains. 50k training data for the target domain would be considered as the in domain data. While training data from the other domains are considered as the out of domain data. Once the data selector is trained, we randomly sample 1M unlabelled data from application traffic, and use data selector to predict, for each data point, the probability of it belonging to the target domain. If the probability is larger than 0.5, we allocate the data point into the SSL data pool for the target domain. To keep the size of SSL data pool consistent across domains, after data selection, we randomly sample 500k for each domain as the final SSL data pool.

\subsubsection{Intelligent Selection of SSL Data}
During the generation of SSL data pool, inclusion of noisy data points, which do not belong to the target domain, are unavoidable. Furthermore, the student-teacher SSL framework is inherently noisy, in that mistakes made by teacher are propagated to the student. Thus, we further explore intelligent data selection methods, aiming to select data points from the SSL data pool, which could facilitate the SSL process more effectively. 

To verify the efficacy of different data selection algorithms, we further apply the data selection approaches on top of the 500k data pool per domain. Here, we compare three approaches, random, submodular optimization and committee filtering. Each method is used to select 300k data from the SSL data pool, which is then used during teacher-student semi-supervised training. 

%\subsection{Experimental Data Sets}
%SNIPS


==> sections/old/intro.tex <==
\label{intro}

% We might not need the fist para as it does not add value. We should add more details to analysis part. 
%Over the last decade, we have seen the advances that deep learning has brought across different fields within the machine learning community. One of the key components that enables neural networks to achieve performance levels that was not possible before is access to large amounts of data. This improvements have been observed across a wide range of machine learning application, such as reinforcement learning (RL) \cite{a3c,alpha_go,dqn}, computer vision (CV) \cite{fast_rcnn,faster_rcnn,yolo,reset}, and natural language processing (NLP) \cite{glove,elmo,bert}. 

Voice-assistants with speech and natural language understanding (NLU) support functionality in multiple domains. For example Google Now, Amazon Alexa and Apple Siri support queries related to music, weather, and others. An NLU system for voice-assistants commonly consists of an intent classifier (IC) and  a named entity recognizer (NER). It takes text input from an automatic speech recognizer (ASR) and predicts intent and entities, which are important information units. For example, if a user asks ``find me a restaurant in new york'', the IC classifies it as SearchPlaceIntent, and the NER classifies ``restaurant'' as PlaceType and ``new york'' as City.

An important requirement for commercial voice-assistants NLU is the ability to continuously add support for new functionalities, i.e., new intents, or new entity types, while improving recognition accuracy for the existing ones. Having high quality labeled data is the key to improve the NLU performance. However, new functionalities often lack labeled data as obtaining human annotation is an expensive process. Furthermore, in the industry setting, in particular when dealing with live systems, we often face the additional challenge of a non-stationary data distribution, given that user behaviors change over time or with trends. In order, to tackle these issues, it is a common practice to continually annotate, and incorporate, new data to the training and test sets, so that as the system evolves the training and test data evolve alongside.  

Obtaining annotations can be an expensive and time-consuming process, so machine learning practitioners often look for ways to minimize the annotation effort. There are two primary approaches to achieve this goal. The first one is Active Learning~\cite{Settles2009ActiveLL} , where the goal is to select a subset of data for annotation such that, when incorporated to the training set, is able to bring the most improvement to the performance of the current model \cite{ralf,coreset,bald,batch_bald}. The second approach is Semi-Supervised Learning which does not require human annotations. Semi-supervised Learning (SSL) provides a framework for utilizing large amount of unlabeled data when obtaining labels are expensive ~\cite{Chapelle2006IntroductionTS}. Contrary to supervised machine learning which relies mainly on labeled data, SSL algorithms can improve model performance by also utilizing unlabeled examples along with the labeled data. SSL techniques have been shown to improve deep models performance across different machine learning tasks including text classification, machine translation, image classification~\cite{cvt,vat,vat_classification}.

A common practice to evaluate SSL algorithms is to take an existing labeled dataset and only use a small fraction of training data as labeled data, while treating the rest of the data as unlabeled dataset. Such evaluation, often constrained to the cases when labelled data is scarce, raises questions about the usefulness of different SSL algorithms in a real-world setting ~\cite{oliver2018realistic}. In particular, unlike widely used NLU datasets such as SNIPS~\cite{Coucke2018SnipsVP}, ATIS~\cite{Price1990EvaluationOS}, internal voice assistant datasets are much bigger and have a lot of redundancy because some queries such as "stop playing", "turn on lights" might be much more frequent that others. In addition, most SSL benchmarks make the assumption that unlabeled dataset comes from the same distribution as the labeled datasets. In voice assistants, this assumption is often violated as by design the labeled dataset also contains synthetic data, crowd-sourced data to represent anticipated usages of a functionality, and unlabeled data doesn't need to follow the same distribution as the labeled data.    


In this paper, we explore different semi-supervised learning techniques that can be leveraged in a large scale industry setting to improve Natural Language Understanding (NLU) tasks. To the best of our knowledge, semi-supervised learning with deep neural networks has not been explored before at this scale for natural language understanding task. In particular, we explore different semi-supervised techniques including pseudo-labeling (PL), knowledge distillation (KD), cross-view training (CVT), and virtual adversarial training (VAT). 

Another unique problem to industry application is the selection of SSL training data from the vast number of unlabeled data, which potentially could be of a different distribution from the labelled data set. Because the distribution and noise level of the SSL training data also impact a model's predictive performance, we further investigate how to effectively select SSL training data from a large pool of data, aiming to optimize training efficiency and model performance. The data selection methods studied are random selection, submodular optimization based selection and committee based selection. 


%These type of techniques are primarily developed in an academic context, and their performance is assessed on standard benchmarks \cite{cifar10,facebook_dataset}. However, in the industry setting, in particular dealing with live systems, we often face added challenge of the distribution of data in which the system is evaluated is non-stationary. More To deal with this problem, it is common practice to continually incorporate, and annotate, new data to the training and test sets, so that as the system evolves the new added data captures the change in distributions. 

% Instead of selecting data for annotation, a machine learning model can be further improved by annotating data according to the current model, or according to some auxiliary model \cite{ssl_vision,mcclosky2006effective}. 

==> sections/old/methods.tex <==
\label{methods}
\subsection{Task Definition}

Intent classification (IC) and named entity recognition (NER) are two important components in natural language understanding (NLU) systems, as well as representatives for two traditional NLP tasks, text classification and sequence tagging. To understand one sentence, we would have to know the intent of that user and the target of that intent. For example, when an user says the sentence, "play welcome to New York", the NLU system has to identify that the intent is "play music", and the target he/she wants is a song named "welcome to New York". The task of identifying the intent is IC while the task of labeling "welcome to New York" as a song name is NER. Our experiments encompass both of these tasks.

\subsection{Model Architecture}

We establish a multi-task LSTM-based model for IC and NER tasks. 300-dimension word embeddings serve as input features. A shared bi-LSTM encoder and two separate task-specific bi-LSTM encoders are applied to encode the sentences. On top of the task-specific encoders, a softmax layer and a conditional random field (CRF) layer are used to decode IC and NER, respectively.

\subsection{Semi-Supervised Learning Approaches}

\subsubsection{SSL Based on Pseudo Label}
Pseudo label (PL) based self-training is a simple and straightforward method of SSL\cite{yarowsky1995unsupervised,mcclosky2006effective}. With this approach, the model's own predictions are used as pseudo labels for the unlabelled data, which is then employed to supplement model training. 

In this study, we first train the IC-NER multi-task model with labelled training data set, denoted as the teacher model. Then we run the teacher model to provide intent and label sequence inferences for the selected unlabelled data pool. Afterwards, a student model is trained with the combined training set of labelled data and data with pseudo labels.     

\subsubsection{SSL Based on Knowledge Distillation}
For Knowledge Distillation (KD) based SSL, a teacher model produces probability distributions over all possible classes and the student model learns from the predicted distribution over labels instead of a predicted label. 

The soft labels on intents are generated by the IC task softmax layer, while the soft labels on label sequences are generated per token, by running softmax on the logits per token before the CRF layer. First a teacher model trained only with labelled data is employed to generate soft labels on selected unlabelled data pool. Then during the training of student model, the labelled data and soft-labelled data are employed to train the model in alternative batches of equal size. For training with soft-labelled data batch, we define the loss as the cross entropy loss between the soft label produced by teacher model and the soft label produced by the student model.    

\subsubsection{Virtual Adversarial Training}
Virtual adversarial training (VAT) is an efficient semi-supervised approach based on adversarial attack \cite{vat}. It whas been shown to be highly effective int both image \cite{vat} and text classifications \cite{vat_classification} tasks. For an unlabelled instance, it generates a small perturbation for the instance that would lead to the largest shift on the label distribution predicted by the model. After getting the adversarial perturbation, the objective is to minimize the KL divergence between the label distribution on the original instance and the instance with perturbation. 

Let $x$ denote an input to the model, $y$ the corresponding label, and $\theta$ the model parameters; the loss, $L$, for VAT can be written as:

\begin{eqnarray}\label{eqn:vat_kl}
    L = KL \big(\hspace{0.1cm} P(\hat{y};x,\hat{\theta})\hspace{0.1cm} ||\hspace{0.1cm} P(\hat{y}; x+d,\hat{\theta})  \big),
\end{eqnarray}

\noindent where $d$ stands for the adversarial perturbation, and $P$ stands for the label distribution for a given input and parameters. The notation  $\hat{y}$ and $\hat{\theta}$ is used to emphasize that the computation of KL divergence takes current estimation of label distribution and parameters.

\subsubsection{Cross-View Training}
Cross-view training (CVT) is another semi-supervised learning approach proved to be efficient on text classification, sequence labeling and machine translation \cite{cvt}. For each time step in a bidirectional LSTM, CVT uses the prediction from the current state as an auxiliary prediction. Then it takes the output from neighbor LSTM neurons for each direction and forces them to predict the same label as the current neuron. 

Denote $f_i$ as the forward output from step $i$ and $b_i$ as the backward output from step $i$. The auxiliary prediction can be written as:

\begin{eqnarray}\label{eqn:cvt_main}
    \hat{y} = Softmax(NN([f_i; b_i]))
\end{eqnarray}

Then $\hat{y}$ would be used as ground truth for 4 adjacent states, and calculate cross entropy (CE) loss:
\begin{eqnarray}\label{eqn:cvt_loss}
    L_{forward} &=& CE(\hat{y}, \hspace{0.1cm}Softmax(NN^{forward}(f_i))) \\
    L_{backward} &=& CE(\hat{y}, \hspace{0.1cm}Softmax(NN^{backward}(b_i))) \\
    L_{past} &=& CE(\hat{y}, \hspace{0.1cm}Softmax(NN^{past}(f_{i-1}))) \\
    L_{future} &=& CE(\hat{y}, \hspace{0.1cm}Softmax(NN^{future}(b_{i+1}))) \\
\end{eqnarray}

The final CVT loss is the mean of them:

\begin{eqnarray}\label{eqn:cvt_total}
    L = \frac{1}{4} * (L_{forward} + L_{backward} + L_{past} + L_{future} )
\end{eqnarray}


\subsection{Data Selection Approaches}

% Data selection problem formulation 
Given a labeled live utterances dataset $D_{labeled}$ and a large unlabled utterances dataset $D_{unlabeled}$, our goal is to select a subset $D_{ssl}\subseteq D_{unlabeled}$ that fits a given budget of utterances to select which can be used for SSL model training. 

\subsubsection{SSL Data Selection using Submodular Optimization}
Submodular optimization is a well studied technique to select a diverse representative subset of a given dataset. Submodular data selection has been applied in speech recognition \cite{wei2015submodularity}, machine translation \cite{kirchhoff2014submodularity} and natural language understanding task~\cite{Cho_2019}. In submodular data selection, submodular functions are chosen to measure the utility of the selected subset. For SSL data selection, we use feature based submodular selection  \cite{kirchhoff2014submodularity}. We use 1-4 ngram as features and use logarithm as a concave function. We filter all n-grams which appear less than $30$ times in $D_{labeled}$ + $D_{unlabeled}$. We use the lazy greedy algorithm to optimize feature-based submodular functions. The algorithm starts with $D_{labeled}$ as the selected data and chooses the utterance from the candidate pool $D_{unlabeled}$ which provides maximum marginal gain. Utterances are selected greedily until the budget constraint is met. 


\subsubsection{SSL Data Filtering by Committee}
Soft labeling techniques tend to work well when the model is able to an accurate prediction on unlabelled data. However, when this is not the case, soft labeling can have a detrimental effect to the overall system, since the model could be providing SSL data that it cannot annotate correctly. Ideally, we would like to have a way of detecting when this might be the case.
Typically, for a given input $x$, neural networks provide a point estimate that is interpreted as a probability distribution over labels; this resulting distribution is highly dependent on several hyper-parameters (i.e., initial parameters, or learning rate). If the point $x$ is easy to learn, neural networks trained from different initial conditions will converge to predicting a similar probability distribution for $x$; on the other hand, if $x$ is difficult to learn, their predicted distribution are likely to disagree or converge to low confidence predictions.

To detect such situations, we train a committee of $n$ teacher models, and compute the entropy of the average probability distribution for every data point. Specifically, we compute the entropy of the average distribution of $x$ as:
\begin{equation}
    H(x) = - \frac{1}{n} \sum_{y \in \mathcal{Y}} \sum_{i=1}^n \Pr(Y=y|X=x,f_i) \log \Pr(Y=y|X=x,f_i)
\end{equation}

Figure \ref{fig:error_rate} shows a visual representation of this phenomenon on three different domains we use in our experiments: Communication, ToDos, Music, and Notifications. The plot shows the error rate (y-axis) in annotation if the model were to predict the label with highest average probability at different levels of entropy (x-axis). For example, for Music, at an entropy level of $0.25$, the committee has an error rate of approximately $5\%$, while at an entropy level of $1.00$, the committee has an error rate over $20\%$.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/fig.png}
    \caption{SSL data annotation by committee error rate as a function of the entropy in the average distribution.}
    \label{fig:error_rate}
\end{figure}

To identify which SSL annotated data we can ``trust'', we train a committee of teacher models, and based on a held-out dataset we identify an entropy level with an acceptable error rate for mis-annotations (e.g., $20\%$). Any SSL annotated data whose entropy level is higher than the identified level, is deemed ``not trustworthy'' and filtered out.





==> sections/old/results.tex <==
\label{results}

\subsection{SSL Techniques}
Table \ref{SSL Comparison} shows the relative error reduction by various SSL techniques, including Pseudo Label (PL),  Knowledge Distillation (KD), Virtual Adversarial Training (VAT) and Cross-View Training (CVT) , over supervised baseline. Also, we report the relative improvement on those SSL techniques with different data selections methods: random selection, submodular optimization based selection, and committee based selection.

From the table \ref{SSL Comparison}, we can summarize that KD is usually better than PL with any specific data selection approach. In addition, CVT and VAT brings large additional gains over KD on both tasks. Between CVT and VAT, CVT usually does better on IC (classification task) and VAT usually brings better performance for NER (sequence labeling task). Moreover, we compare the efficiency between those approaches with the same setting, as shown in the table \ref{SSL Efficiency}. We run each algorithm on Music training data and its randomly selected SSL data, on one Tesla V100 GPU. As suggested in that table, though CVT and VAT brings larger improvement in terms of accuracy, it would also cost more resources to train them. The training time of CVT and VAT is doubled compared to KD and PL. Hence, we should carefully choose the SSL algorithm based on the accuracy target, the task as well as the cost.

% A tradeoff between these two techniques is submodular data selection. \textcolor{red}{Varun, can you add some explanation here?}
% \todo{Varun, can you add some explanation here?}

\begin{table*}[ht]
\caption{\label{SSL Comparison} Error reduction by different SSL methods, relative to baseline. The metric for IC task is intent classification error rate. The metric for NER task is entity recognition F1 error rate.  }
\begin{center}
\small{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\hline 
SSL & Selection & \multicolumn{2}{c|}{Communication} & \multicolumn{2}{c|}{Music} & \multicolumn{2}{c|}{Notifications} & \multicolumn{2}{c}{ToDos} \\ 
\cline{3-10} 
 Algorithm &  Approach & \multicolumn{1}{c|}{IC} & \multicolumn{1}{c|}{NER} & \multicolumn{1}{c|}{IC} & \multicolumn{1}{c|}{NER} & \multicolumn{1}{c|}{IC} & \multicolumn{1}{c|}{NER} &
\multicolumn{1}{c|}{IC} & \multicolumn{1}{c}{NER} \\ \hline 
Baseline &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
PL &  & -3.61\% & -2.86\% & -4.86\% & -3.70\% & -2.79\% & -4.06\% & -2.94\% & -3.33\% \\
KD & Random & -6.35\% & -2.97\% & -6.96\% & -4.40\% & -3.48\% & -4.84\% & -4.18\% & -1.59\% \\
VAT &  & -8.14\% & -8.18\% & -11.15\% & -9.26\% & -6.90\% & -8.55\% & -4.07\% & -4.59\% \\
CVT &  & -9.61\% & -5.26\% & -7.21\% & -8.13\% & -7.39\% & -7.19\% & -4.75\% & -2.38\% \\ \hline 

Baseline &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
PL &  & -4.90\% & -3.11\% &-4.61\% & -3.35\% & -1.48\% & -4.62\% & -1.70\% & -4.32\% \\
KD & Submodular & -6.69\% & -3.40\% & -8.19\% & -3.63\% & -2.91\% & -4.32\% & -5.01\% & -2.59\% \\
VAT &  & -11.56\% & -8.39\% & -14.72\% & -11.03\% & -8.70\% & -11.86\% & -6.24\% & -5.77\% \\
CVT &  & -14.72\% & -5.91\% & -9.84\% & -9.94\% & -8.72\% & -10.61\% & -6.30\% & -3.13\% \\ \hline

Baseline &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
PL &  & -10.54\% & -3.91\% & -9.02\% & -3.93\% & -6.90\% & -4.47\% & -4.55\% & -3.67\% \\
KD & Committee & -11.13\% & -4.46\% & -11.98\% & -4.09\% & -7.76\% & -5.06\% & -6.10\% & -2.61\% \\
VAT &  & -13.16\% & -9.40\% & -13.63\% & -10.10\% & -8.50\% & -11.82\% & -5.75\% & -5.99\% \\
CVT &  & -15.25\% & -6.53\% & -8.72\% & -8.27\% & -8.72\% & -10.40\% & -7.34\% & -3.58\% \\ \hline 
\end{tabular}}
\end{center}
\end{table*}

\begin{table*}[ht]
\caption{\label{SSL Efficiency} Training time for different SSL algorithms on Music with randomly selected SSL data, on one Tesla V100 GPU}
\begin{center}
\small{
\begin{tabular}{c|c|c|c|c}
\hline 
SSL Algorithm & PL & KD & VAT & CVT \\ \hline
Training Time & 30 min & 36 min & 62 min & 75 min \\ \hline

\end{tabular}}
\end{center}
\end{table*}


\subsection{SSL Training Data Set Size}
To investigate how the size of the SSL training data set could impact the performance of the models, we select one of the SSL method, KL based SSL, and carry out a series of experiments on Music domain, with SSL training data set ranging from 10k to 1m, while keeping the labelled data set at 50k size. All training data are randomly selected from the SSL data pool. The results are shown in Table \ref{SSL Data Set Size}. 

It is observed that performance improvement from SSL generally increases with the size of SSL training data set. More SSL training data not only facilitates the transfer of knowledge between teacher and student model, it also exposes the student model to more speech pattern variety from the unlabelled data pool. However, after a certain level, increasing SSL training data size starts to lead to less performance improvement. Because SSL data is labelled using teacher model, it is inherently noisy and contains errors made by the teacher model. When the size of SSL training set is significantly larger than the labelled training set, the noise from teacher labelling could start to dominate the training of student model. Therefore, it is important to maintain a balance between labelled data and SSL training data. 

We observe 500k as an optimal size for SSL training data set, with respect to 50k labelled training data. In the following section, we explore that on top of randomly selected 500k SSL data, how can we further select the data points which are more beneficial to model training, thus improving the training efficiency as well as optimizing the model performance. 

\begin{table*}[ht]
\caption{\label{SSL Data Set Size} For Music domain, using Knowledge Distillation (KL) based SSL, error reduction relative to baseline. The metric for IC task is intent classification error rate. The metric for NER task is entity recognition F1 error rate.  }
\begin{center}
\small{
\begin{tabular}{c|c|c}
\hline 
SSL & \multicolumn{2}{c}{Music}\\ 
\cline{2-3} 
Data Set Size &  \multicolumn{1}{c|}{IC} & \multicolumn{1}{c}{NER} \\ \hline 
10k & -1.07\% & -0.37\% \\ 
50k & -3.81\% & -6.05\% \\ 
100k & -3.37\% & -7.49\% \\
300k & -4.40\% & -6.96\% \\
500k & \textbf{-4.49\%} & \textbf{-8.07\%} \\ 
1m & -4.09\% & -7.20\% \\
\hline

\end{tabular}}
\end{center}
\end{table*}


\subsection{Data Selection Methods}
%\subsubsection{Performance, Efficiency and Data Characteristics}

Table \ref{SSL Comparison} also shows how different data selection techniques affect performance for the SSL methods evaluated. When comparing data selection approaches, we find that there often is a trade-off to be made between computational cost and performance. At one end, random data selection is computationally cheap; we simply uniformly sample a pool of data and use it to generate SSL data, however, we do not have a sense of how helpful or trustworthy that SSL data is. At the other end, data selection by committee is quite expensive; several models need to be trained to generate SSL data. Nontheless, in this case we have a notion of uncertainty for each data point, which prevents poor annotations from harming the classification models. While submodular optimization based selection tries to optimize data selection from diversity aspect, it doesn't filter potentially bad annotation utterances as done in committee based selection. Contrarily, while it's hard to scale committee based selection, submodular optimization based on lazy greedy algorithm provides an scalable solution for a very large unlabeled data pool. 

In order to understand the behavior of different selection algorithms, we compute the unique n-gram ratio present in $\mathcal{D}_l \cup \mathcal{D}_u$ and $\mathcal{D}_l$ data. Table \ref{table:ngram_diversity} shows the unigram and 1-4 gram ratios for different selection algorithm. Unigram ratio of $2$ means that a selection algorithm has expanded the vocabulary size by twice. Similarly 1-4 gram ratio represents the ratio by which ngram vocabulary has expanded. 

\begin{table*}[ht]
\caption{\label{table:ngram_diversity} Unique unigram and 1-4 grams ratio}
\begin{center}
\small{
\begin{tabular}{c|c|c|c|c|c|c}
\hline 
\multirow{2}{*}{Domains} & \multicolumn{2}{c|}{Random} & \multicolumn{2}{c|}{Committee} & \multicolumn{2}{c}{Submod} \\ 
\cline{2-7} 
& \multicolumn{1}{c|}{Unigram} & \multicolumn{1}{c|}{1-4 gram} & \multicolumn{1}{c|}{Unigram} & \multicolumn{1}{c|}{1-4 gram} & \multicolumn{1}{c|}{Unigram} & \multicolumn{1}{c}{1-4 gram} \\ \hline 
Communication & 3.21 &	9.29 &	3.29 & 10.21 & 1.41 & 6.17 \\ 
Todos         & 2.88 &	6.04 &  1.4  & 3.51  & 1.51 & 3.19 \\
Music         & 3.19 &  6.42 &	3.24 & 6.39  & 3.43	& 7.18 \\ 
Notifications & 3.04 &  6.01 &	3.08 & 5.9   & 1.77	& 3.97 \\ 
\hline 
\end{tabular}}
\end{center}
\end{table*}


Within each domain (e.g., Music or Communication) there are several intents representing the goal the user is trying to achieve. A small number of the available intents are used a lot more often than the rest, representing the majority of the data available for training and testing that domain. For example, in the Music domain, the intent PlayMusicIntent, which determines that a user is trying to play a song, is used much more frequently than MusicControlIntent which is used to control volume and other setting for Music.
Given this imbalance in intent distribution, SSL techniques are more likely to result in poor annotations (soft-label or hard-label) for intents that are not encountered very frequently. As such, the performance improvements seen at the domain level might only be the result of improving over-represented intents, or worse, might come at the cost of performance degradation for under represented intents. 

Filtering data based on confidence, as done in KD with committee filtering (KDF), addressed this problem by preventing poor annotation to be included as SSL data. This situation becomes evident from observing table \ref{table:mid-intents}. The table compares the precision (P), recall (R), and f1 score (F1) of under-represented intents; those for which there were between $100$ and $700$ samples. This is in contrast of well represented intents for which we had over $5,000$ samples each.


\begin{table*}[ht]
\caption{\label{table:mid-intents} Performance comparison for mid-size intents for different data filtering methods.  }
\begin{center}
\small{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\hline 
\multirow{2}{*}{Intents} & \multicolumn{3}{c|}{KD} & \multicolumn{3}{c|}{Random} & \multicolumn{3}{c}{KDF} \\ 
\cline{2-10} 
& \multicolumn{1}{c|}{P} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{P} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{P} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c}{F1}   \\ \hline 
CreatePlaylistIntent & 0.59\% & 0.57\% & 0.70\% & 2.75\% & 1.02\% & 1.99\% &5.99\% &1.94\% & \textbf{4.10}\% \\ 
AddToPlaylistIntent &  0.33\% & 1.75\% & 0.99\% & 0.0\% & 1.75\% & 0.77\% & 0.22\% & 2.09\% & \textbf{1.10}\% \\ 
MusicControlIntent & -1.41\% & 3.54\% & 2.30\% & -3.72\% & 5.17\%  & 1.91\%  & -2.04\% & 7.22\% & \textbf{3.32}\% \\
EndCallIntent & 1.37\% & 6.47\% & 1.85\% & 4.40\% & 3.17\% & \textbf{3.84}\% & 9.58\% & -1.91\% & 3.70\% \\ 
GetMessageIntent &  0.32\% & 1.42\% & 0.87\% & 0.65\% & 1.53\% & \textbf{1.09}\% & 0.43\% & 1.42\% & 0.98\% \\ 
BrowseContactList & 1.98\% & 3.33\% & 2.60\% & 2.85\% & 1.97\%  & 2.47\% & 3.22\% & 5.68\% & \textbf{5.94}\% \\
ExtendNotificationIntent & 11.72\% & 26.53\% & 19.11\% & 9.68\% & 30.06\%  & 19.69\% & 19.15\% & 33.34\% & \textbf{26.30}\% \\
EditNotificationIntent & 29.38\% & 29.96\% & 29.79\% & 32.06\% & 31.92\%  & 32.06\% & 34.93\% & 36.33\% & \textbf{35.69}\% \\
EnableNotificationIntent & 21.56\% & 17.87\% & 19.78\% & 24.32\% & 16.81\%  & \textbf{20.62}\% & 22.92\% & 17.52\% & \textbf{20.62}\% \\

\hline 
\end{tabular}}
\end{center}
\end{table*}



\begin{comment}
\begin{table*}[ht]
\caption{\label{Data selection comparison IC} Performance improvement for IC by different SSL methods and different data selection methods, relative to baseline. The metric for IC task is intent classification accuracy. }
\begin{center}
\small{
\begin{tabular}{c|r|r|r|r|r|r|r|r}
\hline 
\multirow{2}{*}{Domains} & \multicolumn{2}{c|}{PL} & \multicolumn{2}{c|}{KD} & \multicolumn{2}{c|}{CVT} & \multicolumn{2}{c|}{VAT} \\ 
\cline{2-9} 
& \multicolumn{1}{c|}{Random} & \multicolumn{1}{c|}{SubM} & \multicolumn{1}{c|}{Random} & \multicolumn{1}{c|}{SubM} & \multicolumn{1}{c|}{Random} & \multicolumn{1}{c|}{SubM} & \multicolumn{1}{c|}{Random} & \multicolumn{1}{c|}{SubM} \\ \hline 
Communication & \\ 
Music & \\ 
Notifications &  \\  \hline 
\end{tabular}}
\end{center}
\end{table*}
\end{comment}




%\subsection{SNIPS Data Set}
